Zero-shot Composed Text-Image Retrieval

In this paper, we consider the problem of composed image retrieval (CIR), it aims to train a model that can fuse multi-modal information, e.g., text and images, to accurately retrieve images that match the query, extending the user's expression ability. We make the following contributions: (i) we initiate a scalable pipeline to automatically construct datasets for training CIR model, by simply exploiting a large-scale dataset of image-text pairs, e.g., a subset of LAION-5B; (ii) we introduce a transformer-based adaptive aggregation model, TransAgg, which employs a simple yet efficient fusion mechanism, to adaptively combine information from diverse modalities; (iii) we conduct extensive ablation studies to investigate the usefulness of our proposed data construction procedure, and the effectiveness of core components in TransAgg; (iv) when evaluating on the publicly available benckmarks under the zero-shot scenario, i.e., training on the automatically constructed datasets, then directly conduct inference on target downstream datasets, e.g., CIRR and FashionIQ, our proposed approach either performs on par with or significantly outperforms the existing state-of-the-art (SOTA) models. Project page: https://code-kunkun.github.io/ZS-CIR/

==> section/03-methods-bak-0504.tex <==
\section{Method}

In this section, we start by formulating the problem of the zero-shot composed image retrieval~(Sec.~\ref{sec:problem}), then describes the procedure for automatically constructing three datasets for CIR task: Laion-CIR-Templates, Laion-CIR-T5 and Laion-CIR-ChatGPT.~(Sec.~\ref{sec:dataset_construction}), lastly, we provide details of our composed image retrieval model~(Sec.~\ref{sec:model}).


\subsection{Problem Scenario}
\label{sec:problem}

\weidi{we need to clearly define the problem here, the following paragraph is not satisfactory.}
To effectively train the CIR model, a significant amount of triplet data is required. Unfortunately, collecting and annotating CIR datasets can be a time-consuming and costly endeavor. To address this, we propose a retrieval-based method that constructs triplets using image text pairs, without the need for manual annotation. 
By using the collected traing set $\mathcal{D}_{train} =\left\{\left( I_{r},I_{t}, t \right)| I_{r} \in \mathbb{R}^{H \times W \times 3}, I_{t} \in \mathbb{R}^{H \times W \times 3}\right\}$, where $I_{r}$ denotes any reference image; $I_{t}$ refers to the target image; $t$ indicates the relative caption. 
Our aim is to develop a fusion network that can successfully generalize to previously \textit{unseen} datasets.


In this paper, we consider the problem of composed image retrieval, 
specifically, given one reference image~($I_r$) and 
conditional description~($t$) that edits the image accordingly, 
our goal is to retrieve the target image~($I_t$) that satisfies the edits. 
\begin{align}
    Q = \Phi_{\text{TBD}}(I_r, t) = \Phi_{\text{AGG}}(\Phi_{\text{FUSE}}(\hspace{1pt} \Phi_{\mathrm{VISUAL-ENC}}\left( I_{r} \right), 
               \hspace{3pt} \Phi_{\mathrm{TEXT-ENC}}\left( t \right) \hspace{1pt}))
\end{align}
where $Q$ refers to the composed query.
Given the composed query, the goal of a retrieval system is to rank all instances in a retrieval set $\Omega = \{I_i, i = 0, \cdots , m\}$ based on their relevance to the query. 
For each query instance pair, the retrieval set is split into the positive
$P_q$ and negative $N_q$ sets, which are formed by the instance that satisfies conditional editing on reference image. 


\weidi{TO CONTINUE ...}
\subsection{Dataset Construction}
\label{sec:dataset_construction}

\begin{figure}
    \centering
    \includegraphics[width=13cm]{images/data_collection.png}
    \caption{Overview of the generation process for CIR triplets. The first row shows three methods of collecting data. Examples of each method are provided on the second row. 
    \weidi{elements in figure are too small, unreadable.}
    % \todo{Need to add some description in Figures or caption to clarify the ``two stages". Besides, you may need to plot the shared 2nd stage corresponding to your paragraph arrangement. See }
    }
    \label{fig:data_collection}
\end{figure}

\revision{We take the \textbf{Laion-COCO} dataset\todo{~\cite{xxx}} that contains the image-caption pairs as our base to generate the CIR triplets. The challenge lies in how to generate a proper relative caption and locate the target image based on the reference image and its caption. To address these issues, we propose two types of approaches, namely, \todo{the template-based method and the model-based method}, both of which consist of the caption-generation stage and the image-retrieval stage as shown in Figure~\ref{fig:data_collection} \todo{It seems that three methods are to relative caption generation, but the target image matching can be shared. }. The details are discussed in the following sections.}

\subsubsection{Template-based approach}
\revision{The template-based approach is to generate the relative caption and target image description based on predefined templates and rules. Here, we consider eight types of semantic operations in the relative caption, namely Cardinality, Addition, Negation, Direct Addressing, Compare\&Change, Comparative Statement, Statement with Conjunction and Viewpoint \todo{it is better to clarify the evidences/reason about our choices. Besides, you can define special font for these operations}. For these operations, it is easy to define some diverse rules and templates edit the original caption of the image in Laion-COCO. Taking the type compare\&change as an example, we first extract the noun phrases from the captions using a part-of-speech (POS) tagger, provided by Spacy\footnote{\href{https://spacy.io/}{https://spacy.io/}}. Then, we can define the template for the relative caption as ``replace \{entity A\} with \{entity B\}'', where the entity A is replaced with other similar noun phrases by using the Sentence-Transformers similarity score. More specifically, we extract the textual feature of noun phrases using the all-MiniLM-L6-v2\footnote{\href{https://huggingface.co/sentence-transformers/all-MiniLM-L6-v2}{https://huggingface.co/sentence-transformers/all-MiniLM-L6-v2}}, and choose an alternative noun phrases whose similarity ranges from 0.5 to 0.7. The target image description is then obtained by replacing entity A with entity B in the reference image description.}

\subsubsection{Language Model-based approach}
\noindent The language model-based approach uses the reference image and the reference image description to allow the language model to directly generate the relative caption and the target image description. More Specifically, we first use the CLIP\cite{radford2021learning} ViT-L/14 image encoder to get the reference image features, convert them into four tokens after a linear layer, and then concatenate with the embedding of reference image description to drive the T5-base\cite{raffel2020exploring} language model to generate the relative caption and target image caption. The model is trained on the clip-filtered-dataset, consisting of 313K triplets created in InstructPix2Pix\cite{brooks2022instructpix2pix}.


\subsubsection{ChatGPT-based approach}
\noindent The ChatGPT-based approach involves providing prompts to ChatGPT in order to generate both a relative caption and a description of the target image directly. For this experiment, the following prompt was used. \weidi{the following English sentence needs to be written properly.}\textit{I have an image. Carefully generate an informative instruction to edit this image content and generate a description of the edited image. I will put my image content beginning with "Image Content:". The instruction you generate should begin with "Instruction:". The edited description you generate should begin with "Edited Description:". The Instruction you generate can cover various semantic aspects, including cardinality, addition, negation, direct addressing, compare\&change, comparative, conjunction, spatial relations\&background, viewpoint. The edited description need to be as simple as possible. The instruction does not need to explicitly indicate which type it is. Avoid adding imaginary things. "Image Content: \{\}". Each time generate one instruction and one edited description only.}
\weidi{I don't understand this, do you mean: ``provide the caption of reference image to chatGPT, and ask it to edit this sentence, and output the caption for target image'' ?}

\vspace{5pt}
\subsubsection{Retrieval Details}
\noindent The study focuses on the initial one million data entries from the Laion-COCO dataset. The caption features of Laion-COCO are extracted using the all-MiniLM-L6-v2 Model as a first step. We then employ the faiss package to perform similarity retrieval once we have the generated target image description. Images with a similarity exceeding the threshold are retained, whereas those with less are discarded.


\subsection{Composed Image Retrieval Model}
\label{sec:model}

\begin{figure}
    \centering
    \includegraphics[width=13cm]{images/model.png}
    \caption{Overview of our proposed model, which consists of a visual and text encoder, a Transformer module and a dynamic aggregation module. \jiangchao{Interaction might be more accurate than ''fusion" about the role of Transformer based on its IO in the above illustration. dynamic aggregation is not better than ``adaptive aggregation".}}
    \label{fig:architecture}
\end{figure}
\weidi{give an high-level sentence to describe what will be included in this section, {\em e.g.}, architecture design, training procedure.}

\noindent \revision{In this part, we present the architecture of our CIR model in Section \ref{sec:arch} and describe its training in Section \ref{sec:training_procedure}. }
% Figure \ref{fig:architecture} gives an overview of the model.

\subsubsection{Architecture} \label{sec:arch}
\revision{The proposed CIR Model is illustrated in Figure \ref{fig:architecture}, which consists of three components: the encoders to extract features from visual data and textual data respectively, a Transformer module to capture the high-order interaction between two modalities, and an adaptive aggregation to fuse all features together. We introduce the details of each component as follows.}

\vspace{5pt}
\noindent \textbf{Visual and Text Encoders.} \revision{We adopt pre-trained vision and language models as our encoders for different modalities given their impressive performance and flexibility to maintain the semantics. Formally, we denote the feature extraction via the following notations,}
% \begin{align}\label{eq:encoders}
% \begin{split]
% & \mathcal{F}_{\mathrm{V}} =\Phi_{\mathrm{VISUAL-ENC}}\left( I_{ref} \right)\in \mathbb{R}^{|\mathcal{V}| \times d} \\
% & \mathcal{F}_{\mathrm{W}} =\Phi_{\mathrm{TEXT-ENC}}\left( T \right)\in \mathbb{R}^{|\mathcal{W}| \times d}
% \end{split}
% \end{align}
\begin{align}
    \begin{split}
        & \mathcal{F}_{\mathrm{V}} =\Phi_{\mathrm{VISUAL-ENC}}\left( I_{r} \right)\in \mathbb{R}^{|\mathcal{V}| \times d}, \qquad \mathcal{F}_{\mathrm{W}} =\Phi_{\mathrm{TEXT-ENC}}\left( t \right)\in \mathbb{R}^{|\mathcal{W}| \times d}, 
    \end{split}
\end{align}
\noindent \revision{where $I_{ref}$ denotes the query image encoded by the visual encoder $\Phi_{\mathrm{VISUAL-ENC}}$, and $t$ refers to the editing text encoded by the textual encoder $\Phi_{\mathrm{TEXT-ENC}}$. In the experiments, we primarily consider the pretrained BLIP~\cite{li2022blip} and CLIP~\cite{radford2021learning} as our visual and text encoders.}

\vspace{5pt}
\noindent \textbf{The Transformer module.} \revision{Regarding the input of our Transformer module, except $\mathcal{F}_{\mathrm{V}}$ and $\mathcal{F}_{\mathrm{W}}$, a learnable token embedding $ \mathcal{F}_{\mathrm{Sep}} $ is integrated to better discriminate the characteristics of various modalities. The feature interaction between the visual modality and the textual modality together with a separate token is then formulated in the following.}
\begin{equation}
\left[\mathcal{F}_{\mathrm{V}}^{\prime}, \mathcal{F}_{\mathrm{Sep}}^{\prime}, \mathcal{F}_{\mathrm{W}}^{\prime}\right]=\Phi_{\mathrm{FUSE}}\left(\left[\mathcal{F}_{\mathrm{V}}, \mathcal{F}_{\mathrm{Sep}}, \mathcal{F}_{\mathrm{W}}\right]\right)
\end{equation}

\noindent \revision{where $[\cdot, \cdot, \cdot]$ denotes the feature concatenation, $\Phi_{\mathrm{FUSE}}$ is the two-layer Transformer module, and the input and the output of each feature vector maintains the same shape. The visual feature $\mathcal{F}_{\mathrm{V}}$ and the textual feature $\mathcal{F}_{\mathrm{W}}$ have been augmented through the feature interaction in the Transformer, resulting in the refined features $\mathcal{F}_{\mathrm{V}}^{\prime}$ and $\mathcal{F}_{\mathrm{W}}^{\prime}$. \todo{How $ \mathcal{F}_{\mathrm{Sep}} $ works in this process should be specially discussed here.}}

\vspace{5pt}
\noindent \textbf{Adaptive Aggregation.} 
\revision{After obtaining $ \mathcal{F}_{\mathrm{V}}^{\prime} \in \mathbb{R}^{|\mathcal{V}| \times d} $ and $ \mathcal{F}_{\mathrm{W}}^{\prime} \in \mathbb{R}^{|\mathcal{W}| \times d} $, we take out the internal features corresponding to the image global patch and the text global token respectively, and concatenate them together to be transformed as the fusion features $ \mathcal{F}_{\mathrm{U}}\in \mathbb{R}^{d}$ through an MLP module. On top of $ \mathcal{F}_{\mathrm{U}} $, a simple but effective adaptive fusion is proposed. Specifically, we apply a linear layer to project $ \mathcal{F}_{\mathrm{U}} $ into three weight parameters ($w_1, w_2, w_3$) that act as multipliers for $ \mathcal{F}_{\mathrm{V}}^{\mathrm{G}}$, $ \mathcal{F}_{\mathrm{U}} $ and $ \mathcal{F}_{\mathrm{W}}^{\mathrm{G}}$. The $ \mathcal{F}_{\mathrm{V}}^{\mathrm{G}}$ indicates the global BLIP/CLIP visual features and the $ \mathcal{F}_{\mathrm{W}}^{\mathrm{G}}$ denotes the global BLIP/CLIP textual features. The final image-text representation $Q$ is computed as:}
\begin{equation}
\label{eq:Q}
    Q = w_1 * \mathcal{F}_{\mathrm{V}}^{\mathrm{G}} + w_2 * \mathcal{F}_{\mathrm{U}} + w_3 * \mathcal{F}_{\mathrm{W}}^{\mathrm{G}}
\end{equation}


\subsubsection{The Training Objective}
\label{sec:training_procedure}
\textbf{Training on Our Collected CIR Dataset.} We follow previous work and use the batch-based classification (BBC) loss\todo{~\cite{vo2019composing}}. \revision{Given a batch size of $B$, the $i$-th query pair ($I_R^i, t^i$) should be close to its positive target $I_T^i$ and far away from the negative targets, which can be formulated as}
\begin{equation}
\mathcal{L}=-\frac{1}{B} \sum_{i=1}^B \log \left[\frac{\exp \left[\lambda \cdot \kappa\left(Q, I_{\mathrm{T}}^i\right)\right]}{\sum_{j=1}^B \exp \left[\lambda \cdot \kappa\left(Q, I_{\mathrm{T}}^j\right)\right]}\right],
\end{equation}
\noindent \revision{where $\lambda$ is the temperature parameter that is set to 100 following~\cite{baldrati2022conditioned}, and $\kappa(\cdot,\cdot)$ denotes the cosine similarity, and $Q$ is computed by Eq.\eqref{eq:Q}.} 
% \todo{(1) Fix the notations. (2) directly use $\mathcal{F}$ for the fusion and (3) explain $\mathcal{F}$ that is computed by Eq.xx and Eq. xx.}

==> section/experiment-backup.tex <==
\section{Experiment}
%\weidi{TO CONTINUE .....}

\subsection{Experimental Setups}
\noindent \textbf{Training Datasets.}
We construct the training sets by using the data collection pipeline outlined in Section~\ref{sec:dataset_construction},
resulting Laion-CIR-Template and Laion-CIR-LLM,
depending on the adopted approaches.
%We have categorized the collected datasets based on the different approaches and refer to them as Laion-CIR-Template and Laion-CIR-LLM. 
Laion-CIR-Template contains 16000 triplets and Laion-CIR-LLM consists of 15033 triplets, respectively.

\vspace{3pt}
\noindent \textbf{Evaluation Datasets.} 
We evaluate our model on two public benchmarks, namely, CIRR~\cite{liu2021image} and FashionIQ~\cite{wu2021fashion}. \textit{CIRR} comprises approximately 36K triplets that were sampled from generic images obtained from $\rm NLVR^2$\cite{suhr2018corpus}. 
To mitigate the false negative case, the author conducted two benchmarks to demonstrate fine-grained retrieval. The first benchmark involved a general search using the entire validation corpus as the target search space. The second benchmark focused on a subset of six images similar to the query image, based on pre-trained ResNet15 feature distance. \textit{FashionIQ} focus on fashion domain and is divided into three sub categories, \textit{Dress, Shirt and Toptee.} It contains more than 30k triplets. The reference and target images were matched based on similarities in their titles, and each triplets was accompanied by two annotations that were manually generated by human annotators.
{\bf Note that}, in this paper, we consider zero-shot evaluation, 
that is to say, we only train on our automatically constructed training set, and directly evaluating on the target benchmarks.

\vspace{3pt}
\noindent \textbf{Evaluation Metrics.} 
We adopt standard metric in retrieval, {\em i.e.}, $\rm Recall@K$, which denotes the percentage of target images being included in the top k list. For CIRR dataset, we also report $\rm Recall_{Subset}@K$ metric, which considers only the images within the subset of the query.


\subsection{Implementation Details}

Our framework is implemented with PyTorch, 
and all experiments are conducted on 24G GeForce RTX 3090 GPU. 
Following CLIP4CIR~\cite{baldrati2022conditioned}, 
we use the targetpad as our image processor. 
\weidi{what is targetpad ?}
The transformer-based fusion module contains 2 layers with 8 heads. 
We adopt AdamW optimizer, using a learning rate of $10^{-4}$ with a cosine decay schedule. 
For visual encoder, we use pre-trained BLIP~\cite{li2022blip} w/ViT-B. %that has undergone image-text retrieval fine-tuning on COCO~\cite{lin2014microsoft} dataset.
\weidi{what about CLIP model ?}


\weidi{what does this belong to ? for the language model used in template-based dataset construction ? give more detail on it.}
More specifically, we extract the textual feature of noun phrases using the all-MiniLM-L6-v2\footnote{\href{https://huggingface.co/sentence-transformers/all-MiniLM-L6-v2}{https://huggingface.co/sentence-transformers/all-MiniLM-L6-v2}}, and choose an alternative noun phrase whose similarity ranges from 0.5 to 0.7. 



\subsection{Ablation Study}
In this section, we conducted experiments on different pre-trained backbones and fine-tuning types to access the generalizability of our data collection method. Additionally, we performed ablation experiments to determine the importance of each components in our CIR model, focusing specifically on the transformer-based fusioner and dynamic aggregation.

\subsubsection{Different Pre-trained Backbone and Fine-tuning Type}
Our study results indicate that the model performs effectively under both the CLIP\cite{radford2021learning} and BLIP\cite{li2022blip} architectures as demonstrated in tables \ref{table:ablation_cirr} and \ref{table:ablation_fiq}. We can see that using a larger, better model and fine tuning more parameters tends to give better results. It is worth mentioning that our model has achieved comparable or even better performance than some recent works under the CLIP architecture.
% Specifically, our approach surpasses other methods that employ CLIP as the backbone, achieving better results in various metrics of the CIRR dataset, as well as the FashionIQ recall@50 metric.

\begin{table}
\centering
\footnotesize
\begin{tabular}{c c||c|c|c|c|c|c|c}
\hline
 \multicolumn{2}{c||}{~}&
 \multicolumn{4}{c|}{\text{$\rm Recall@K$}}& 
 \multicolumn{3}{c}{\text{$\rm Recall_{Subset}@K$}} \\
 Backbone&Fine-tuning Type& K=1& K=5& K=10& K=50& K=1& K=2& K=3\\
 \hline \hline
 \multirow{3}{5em}{CLIP-B/32} & Freeze & 24.46 & 53.61 & 67.54 & 89.81 & 57.81 & 78.17 & 89.54\\
 &Text encoder &27.08 &57.21 &70.31 &90.39&62.70 &82.41 &92.15\\
 &Both&29.30 &60.48 &73.25&92.31&63.57 &82.31 &91.95\\
 \hline
 \multirow{2}{5em}{CLIP-L/14} & Freeze & 25.04 & 53.98 & 67.59 & 88.94 & 55.33 & 76.82 & 88.94\\ 
 &Text encoder &27.90 &58.27 &71.01 &91.30&60.48 &80.31 &90.75\\
 \hline
\multirow{2}{3em}{BLIP}& Freeze & 34.89 & 64.75 & 76.24 & 92.22 & 66.34 & 83.76 & 92.92\\ 
& Text encoder & 38.43 & 68.92 & 79.93 & 94.05 & 68.60 & 85.61 & 93.93\\
 \hline
\end{tabular}
\caption{Generalization for different backbones and fine-tuning types on CIRR. Freeze means the entire pre-trained model is frozen. Text encoder means only the text encoder is fine-tuned. Both means the entire pre-trained model is fine-tuned.}
\label{table:ablation_cirr}
\end{table}

\begin{table}
\begin{scriptsize}
\centering
\begin{tabular}{c c||c c|c c|c c|c c}
\hline
 \multicolumn{2}{c||}{~}&
 \multicolumn{2}{c|}{Shirt}& 
 \multicolumn{2}{c|}{Dress}& 
 \multicolumn{2}{c|}{TopTee}&
 \multicolumn{2}{c}{Average}\\
 Backbone & Fine-tuning Type& \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50}\\
 \hline \hline
 \multirow{3}{5em}{CLIP-B/32} & Freeze & 25.37 & 42.69 & 19.44 & 42.04 & 26.93 & 49.31 & 23.91& 44.68\\ 
 &Text encoder&27.38 & 45.58 & 21.47 & 43.88 & 28.15 & 49.82 & 25.67 & 46.43\\
 &Both&27.48&46.52&20.58&43.28&27.38&48.50&25.15&46.10\\
 \hline
 \multirow{2}{5em}{CLIP-L/14} & Freeze & 29.54 & 47.79 & 23.85 & 44.57 & 32.33 & 52.52 & 28.57& 48.29\\ 
 &Text encoder &30.91 &49.31&27.32 &47.79&33.61 &54.05 &30.61& 50.38\\
 \hline
 \multirow{2}{3em}{BLIP} & Freeze & 28.07 & 45.63 & 21.67 & 41.89 & 31.11 & 50.79 & 26.95& 46.10\\ 
 &Text encoder &32.83 &52.40&27.86 &49.48&35.24 &57.42 &31.98& 53.10\\
 \hline
\end{tabular}
\caption{Generalization for different backbones and fine-tuning types on FashionIQ. Freeze means the entire pre-trained model is frozen. Text encoder means only the text encoder is fine-tuned. Both means the entire pre-trained model is fine-tuned.}
\label{table:ablation_fiq}
\end{scriptsize}
\end{table}

\subsubsection{Effect of Individual Modules in our CIR Model}
To investigate the importance of each component in our CIR model, we conduct ablation experiments on the transformer-based fusioner and the dynamic aggregation, and change one variable at a time. The experiments are conducted using the model trained on Laion-CIR-ChatGPT in Table \ref{table:sota_fiq}. Table \ref{table:ablation_component_fiq} illustrates that replacing dynamic aggregation with learnable weights results in a significant decrease in performance, which could be due to the distribution differences between the training and test sets. Using static aggregation may result in a decline in the overall generalization ability of the model, especially in a testing scenario. Not implementing fusioner to integrate the information from different modalities leads to a decrease in performance metrics. Demonstrating the crucial role of multi-modal information integration.

% \begin{table}
% \begin{scriptsize}
% \centering
% \begin{tabular}{c c||c c|c c|c c|c c}
% \hline
%  \multicolumn{2}{c||}{~}&
%  \multicolumn{2}{c|}{Shirt}& 
%  \multicolumn{2}{c|}{Dress}& 
%  \multicolumn{2}{c|}{TopTee}&
%  \multicolumn{2}{c}{Average}\\
%  Fusioner & Aggregation& \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50}\\
%  \hline \hline
%  \ding{52} & \ding{56} & 30.57 & 50.34 & 26.57 & 48.64 & 33.81 & 53.70 & 30.32& 50.89\\ 
%  \ding{56} & \ding{52}&31.40 & 51.42 & 26.92 & 48.34 & 35.19 & 56.15 & 31.17 & 51.97\\
%   \ding{52} & \ding{52}&32.24 & 52.06 & 28.90 & 49.43 & 36.56 & 58.49 & 32.60 & 53.33\\
%  \hline
% \end{tabular}
% \caption{Ablation study on FashionIQ}
% \label{table:ablation_component_fiq}
% \end{scriptsize}
% \end{table}
\begin{table}
\begin{tiny}
\setlength{\tabcolsep}{0.12cm}
\centering
\begin{tabular}{c c c c|c c|c c|c c|c c}
\hline
 \multicolumn{4}{c|}{~}&
 \multicolumn{2}{c|}{Shirt}& 
 \multicolumn{2}{c|}{Dress}& 
 \multicolumn{2}{c|}{TopTee}&
 \multicolumn{2}{c}{Average}\\
 Method & Fine-tuning Type & Fusioner & Aggregation& \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50}\\
 \hline \hline
 Template-based & freeze & \ding{52} & \ding{56} & 25.22 & 42.89 & 19.88 & 40.16 & 26.77 & 46.81 & 23.96& 43.29\\ 
 Template-based & freeze & \ding{56} & \ding{52}&27.43 & 45.24 & 22.21 & 41.40 & 29.07 & 51.66 & 26.24 & 46.10\\
 Template-based & freeze & \ding{52} & \ding{52}&28.07 & 45.63 & 21.67 & 41.89 & 31.11 & 50.79 & 26.95 & 46.10\\
 \hline
 Template-based & text encoder & \ding{52} & \ding{56} & 33.56 & 52.70 & 27.17 & 50.03 & 35.75 & 56.35 & 32.16& 53.03\\ 
 Template-based & text encoder & \ding{56} & \ding{52}&33.12 & 52.80 & 29.20 & 50.22 & 35.90 & 58.80 & 32.74 & 53.94\\
 Template-based & text encoder & \ding{52} & \ding{52}&32.83 & 52.40 & 27.86 & 49.48 & 35.24 & 57.42 & 31.98 & 53.10\\
 \hline
 LLM-based & freeze & \ding{52} & \ding{56} & 21.98 & 39.35 & 18.10 & 38.42 & 23.51 & 43.65 & 21.20& 40.47\\ 
 LLM-based & freeze & \ding{56} & \ding{52}&28.46 & 47.79 & 25.04 & 45.41 & 31.67 & 52.98 & 28.39 & 48.73\\
 LLM-based & freeze & \ding{52} & \ding{52}&31.89 & 50.25 & 27.07 & 47.89 & 35.39 & 56.40 & 31.45 & 51.51\\
 \hline
 LLM-based & text encoder & \ding{52} & \ding{56} & 30.57 & 50.34 & 26.57 & 48.64 & 33.81 & 53.70 & 30.32& 50.89\\ 
 LLM-based & text encoder & \ding{56} & \ding{52}&31.40 & 51.42 & 26.92 & 48.34 & 35.19 & 56.15 & 31.17 & 51.97\\
 LLM-based & text encoder & \ding{52} & \ding{52}&32.24 & 52.06 & 28.90 & 49.43 & 36.56 & 58.49 & 32.60 & 53.33\\
 \hline
\end{tabular}
\caption{Ablation study on FashionIQ}
\label{table:ablation_component_fiq}
\end{tiny}
\end{table}




% \begin{table}
% \footnotesize
% \begin{tabular}{c c||c|c|c|c|c|c|c}
% \hline
%  \multicolumn{2}{c||}{~}&
%  \multicolumn{4}{c|}{\text{$Recall@K$}}& 
%  \multicolumn{3}{c}{\text{$Recall_{Subset}@K$}} \\
%  Backbone&Method& K=1& K=5& K=10& K=50& K=1& K=2& K=3\\
%  \hline \hline
%  \multirow{9}{0em}{B/32} & Image-only & 6.89 & 22.99 & 33.68 & 59.23 & 21.04 & 41.04 & 60.31\\
%  &Text-only &21.81 &45.22 &57.42 &81.01&62.24 &81.13 &90.70\\
%  &Image + Text&11.71 &35.06 &48.94 &77.49&32.77 &56.89 &74.96\\
%  &PALAVRA&16.62 &43.49 &58.51 &83.95&41.61 &65.30 &80.94\\
%  &SEARLE-OTI &24.27 &53.25 &66.10 &88.84&54.10 &75.81 &87.33\\
%  &SEARLE &23.57 &52.80 &66.48 &89.59&54.80 &76.70 &88.10\\
%  &\textbf{Template-based} &29.30 &60.48 &73.25 &92.31&63.57 &82.31 &91.95\\
%  &\textbf{Language Model-based} &28.55 &59.64 &72.27 &92.43&57.83 &78.77 &90.07\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x &x\\
%  \hline
%  \multirow{7}{0em}{L/14} & Pic2Word & 23.90 & 51.70 & 65.30 & 87.80 & - & - & -\\ 
%  &SEARLE-XL-OTI &24.87 &52.31 &66.29 &88.58&53.80 &74.31 &86.94\\
%  &SEARLE-XL &24.22 &52.41 &66.29 &88.63&53.71 &74.63 &87.61\\
%  &CompoDiff&18.24 &53.14 &70.82 &90.35&27.51 &48.30 &65.54\\
%  &\textbf{Template-based}&28.05 & 56.99 &70.31 & 90.34 & 57.37 & 78.39& 89.13\\
%  &\textbf{Language Model-based}&27.37 & 57.52 &70.22 & 90.72 & 57.06 & 77.13& 89.54\\
%  &\textbf{ChatGPT-based}&x & x &x & x & x & x& x\\
%  \hline
% \multirow{4}{0em}{BLIP}& CASE Pre-LaSCo.Ca. & 35.40 & 65.78 & 78.53 & 94.63 & 64.29 & 82.66 & 91.61\\ 
% & \textbf{Template-based} & 38.43 & 68.92 & 79.93 & 94.05 & 68.60 & 85.61 & 93.93\\ 
% & \textbf{Language Model-based} & 36.53 & 67.59 & 79.13 & 94.36 & 64.72 & 82.80 & 92.22\\ 
%  & \textbf{ChatGPT-based} & 36.82 & 66.65 & 78.55 & 93.57 & 64.60 & 82.94 & 92.27\\ 
%  \hline
% \end{tabular}
% \caption{Comparision on CIRR test set.}
% \label{table:sota_cirr}
% \end{table}


% \begin{table}
% \begin{scriptsize}
% \centering
% \begin{tabular}{c c||c c|c c|c c|c c}
% \hline
%  \multicolumn{2}{c||}{~}&
%  \multicolumn{2}{c|}{Shirt}& 
%  \multicolumn{2}{c|}{Dress}& 
%  \multicolumn{2}{c|}{TopTee}&
%  \multicolumn{2}{c}{Average}\\
%  Backbone & Method& \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50}\\
%  \hline \hline
%  \multirow{9}{0em}{B/32} & Image-only & 6.92 & 14.23 & 4.46 & 12.19 & 6.32 & 13.77 & 5.90& 13.37\\ 
%  &Text-only&19.87 & 34.99 & 15.42 & 35.05 & 20.81 & 40.49 & 18.70 & 36.84\\
%  &Image + Text&13.44&26.25&13.83&30.88&17.08&31.67&14.78&29.60\\
%  &PALAVRA&21.49&37.05&17.25&35.94&20.55&38.76&19.76&37.25\\
%  &SEARLE-OTI&25.37&41.32&17.85&39.91&24.12&45.79&22.44&42.34\\
%  &SEARLE & 24.83 & 41.11 & 18.15 & 38.57 & 25.60&46.25&22.86&41.98\\
%  &\textbf{Template-based} & 27.48 & 46.52 & 20.58 & 43.28 & 27.38 & 48.50 & 25.15 & 46.10\\
%  &\textbf{Language Model-based} & 26.74 & 47.06 & 22.81 & 44.62 & 29.07 & 49.62 & 26.21 & 47.10\\
%  &\textbf{ChatGPT-based} & x & x & x & x & x & x & x & x\\
%  \hline
%  \multirow{7}{0em}{L/14} & Pic2Word & 26.20 & 43.60 & 20.00 & 40.20 & 27.90 & 47.40 & 24.70& 43.70\\ 
%  &SEARLE-XL-OTI &30.37 &47.49&21.57 &44.47&30.90 &51.76 &27.61& 47.90\\
%  &SEARLE-XL &27.43 &45.68&20.32 &43.18&29.32 &50.17 &25.69& 46.34\\
%  &CompoDiff &37.69 &49.08&32.24 &46.27&38.12 &50.57 &36.02& 48.64\\
%  &\textbf{Template-based} &30.91 &49.31 &27.32 &47.79&33.61 &54.05&30.61&50.38\\
%  &\textbf{Language Model-based} &31.26 &50.44 &24.54 &45.61&32.48 &54.41&29.43&50.15\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x&x&x\\
%  \hline
% \end{tabular}
% \caption{Comparasion on FashionIQ validation set.}
% \label{table:sota_fiq}
% \end{scriptsize}
% \end{table}


% \begin{table}
% \centering
% \begin{footnotesize}
% \begin{tabular}{c c||c|c|c|c|c|c|c}
% \hline
%  \multicolumn{2}{c||}{~}&
%  \multicolumn{4}{c|}{\text{$Recall@K$}}& 
%  \multicolumn{3}{c}{\text{$Recall_{Subset}@K$}}\\
%  Fine-tuning Type&Method& K=1& K=5& K=10& K=50& K=1& K=2& K=3\\
%  \hline \hline
%  \multirow{3}{6em}{Freeze CLIP} 
%  &\textbf{Template-based} &24.46 &53.61 &67.54 &89.81&57.81 &78.17 &89.54\\
%  &\textbf{Language Model-based} &23.49 &52.05 &65.76 &88.82&55.25 &76.58 &89.04\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x &x\\
%  \hline
%  \multirow{3}{6em}{Finetune CLIP Text}
%  &\textbf{Template-based}&27.08 & 57.21 &70.31 & 90.39 & 62.70 & 82.41& 92.15\\
%  &\textbf{Language Model-based}&26.43 & 56.27 &69.11 & 90.17 & 58.10 & 79.47& 89.88\\
%  &\textbf{ChatGPT-based}&x & x &x & x & x & x& x\\
%  \hline
%  \multirow{3}{6em}{Finetune CLIP Both}
%  &\textbf{Template-based}&29.30 & 60.48 &73.25 & 92.31 & 63.57 & 82.31& 91.95\\
%  &\textbf{Language Model-based}&28.55 & 59.64 &72.27 & 92.43 & 57.83 & 78.77& 90.07\\
%  &\textbf{ChatGPT-based}&x & x &x & x & x & x& x\\

%  \hline
% \end{tabular}
% \caption{ViT-B/32 | CIRR}
% \end{footnotesize}
% \end{table}

% \begin{table}
% \centering
% \begin{footnotesize}
% \begin{tabular}{c c||c|c|c|c|c|c|c}
% \hline
%  \multicolumn{2}{c||}{~}&
%  \multicolumn{4}{c|}{\text{$Recall@K$}}& 
%  \multicolumn{3}{c}{\text{$Recall_{Subset}@K$}}\\
%  Fine-tuning Type&Method& K=1& K=5& K=10& K=50& K=1& K=2& K=3\\
%  \hline \hline
%  \multirow{3}{6em}{Freeze CLIP} 
%  &\textbf{Template-based} &25.04 & 53.98 &67.59 & 88.94 & 55.33 & 76.82& 88.94\\
%  &\textbf{Language Model-based}&22.46 & 51.47 &65.33 & 88.19 & 49.16 & 72.00& 86.48\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x &x\\
%  \hline
%  \multirow{3}{6em}{Finetune CLIP Text}
%  &\textbf{Template-based}&27.90 &58.27 &71.01 &91.30&60.48 &80.31 &90.75\\
%  &\textbf{Language Model-based}&26.31 & 56.48 &68.58 & 89.66 & 56.58 & 77.08& 89.59\\
%  &\textbf{ChatGPT-based}&x & x &x & x & x & x& x\\
%  \hline
%  \multirow{3}{6em}{Finetune CLIP Both}
%  &\textbf{Template-based}&x & x &x & x & x & x& x\\
%  &\textbf{Language Model-based}&x & x &x & x & x & x& x\\
%  &\textbf{ChatGPT-based}&x & x &x & x & x & x& x\\

%  \hline
% \end{tabular}
% \caption{ViT-L/14 | CIRR}
% \end{footnotesize}
% \end{table}

% \begin{table}
% \centering
% {\scriptsize
% \begin{tabular}{c c||c c|c c|c c|c c}
% \hline
%  \multicolumn{2}{c||}{~}&
%  \multicolumn{2}{c|}{Shirt}& 
%  \multicolumn{2}{c|}{Dress}& 
%  \multicolumn{2}{c|}{TopTee}&
%  \multicolumn{2}{c}{Average}\\
%  Fine-tuning Type& Method& \text{R@10}& \text{R@50}& \text{R@10}& \text{R@50}& \text{R@10}& \text{R@50}& \text{R@10}& \text{R@50}\\
%  \hline \hline
%  \multirow{3}{6em}{Freeze CLIP} &\textbf{Template-based} &25.37 &42.69 &19.44 &42.04&26.93 &49.31&23.91&44.68\\
%  &\textbf{Language Model-based} &24.10 &39.60 &18.34 &40.01&26.93 &45.54&23.12&41.72\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x&x&x\\
%  \hline
%  \multirow{3}{6em}{Finetune CLIP Text} &\textbf{Template-based} & 27.38 & 45.58 & 21.47 & 43.88 & 28.15 & 49.82 & 25.67 & 46.43\\
%  &\textbf{Language Model-based} & 26.30 & 44.85 & 20.63 & 43.83 & 28.61 & 50.28 & 25.18 & 46.32\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x&x&x\\
%  \hline
%  \multirow{3}{6em}{Finetune CLIP Both} &\textbf{Template-based} &27.48 &46.52 &20.58 &43.28&27.38 &48.50&25.15&46.10\\
%  &\textbf{Language Model-based} &26.74 &47.06 &22.81 &44.62&29.07 &49.62&26.21&47.10\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x&x&x\\
%  \hline
% \end{tabular}}
% \caption{ViT-B/32 | FashionIQ}
% \end{table}

% \begin{table}
% \centering
% {\scriptsize
% \begin{tabular}{c c||c c|c c|c c|c c}
% \hline
%  \multicolumn{2}{c||}{~}&
%  \multicolumn{2}{c|}{Shirt}& 
%  \multicolumn{2}{c|}{Dress}& 
%  \multicolumn{2}{c|}{TopTee}&
%  \multicolumn{2}{c}{Average}\\
%  Fine-tuning Type& Method& \text{R@10}& \text{R@50}& \text{R@10}& \text{R@50}& \text{R@10}& \text{R@50}& \text{R@10}& \text{R@50}\\
%  \hline \hline
%  \multirow{3}{6em}{Freeze CLIP} &\textbf{Template-based} &29.54 &47.79 &23.85 &44.57&32.33 &52.52&28.57&48.29\\
%  &\textbf{Language Model-based} &28.17 &46.47 &22.06 &41.60&31.36 &49.98&27.20&46.02\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x&x&x\\
%  \hline
%  \multirow{3}{6em}{Finetune CLIP Text} &\textbf{Template-based} &30.91 &49.31 &27.32 &47.79&33.61 &54.05&30.61&50.38\\
%  &\textbf{Language Model-based} &31.94 &50.10 &23.55 &45.96&33.66 &54.72&29.72&50.26\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x&x&x\\
%  \hline
%  \multirow{3}{6em}{Finetune CLIP Both} &\textbf{Template-based} &x &x &x &x&x &x&x&x\\
%  &\textbf{Language Model-based} &x &x &x &x&x &x&x&x\\
%  &\textbf{ChatGPT-based} &x &x &x &x&x &x&x&x\\
%  \hline
% \end{tabular}}
% \caption{ViT-L/14 | FashionIQ}
% \end{table}





% \begin{figure}[htbp]
% \centering

% \subfigure[Template-based]{
% \begin{minipage}[t]{0.3\linewidth} %linewidth小于0.5
% \centering
% \includegraphics[width=1.5in]{images/qualitative1.png} 
% %\caption{fig1}
% \end{minipage}%
% }%
% \subfigure[Language Model-based]{
% \begin{minipage}[t]{0.3\linewidth} %linewidth小于0.5
% \centering
% \includegraphics[width=1.5in]{images/qualitative2.png}
% %\caption{fig2}
% \end{minipage}%
% }%
% \subfigure[ChatGPT-based]{
% \begin{minipage}[t]{0.3\linewidth} %linewidth小于0.5
% \centering
% \includegraphics[width=1.5in]{images/qualitative3.png}
% %\caption{fig2}
% \end{minipage}%
% }%

% \centering
% \caption{Qualitative Results}
% \end{figure}


\subsection{Comparison with State-of-the-art}
We compare our method with various zero-shot composed image retrieval methods on CIRR and FashionIQ. As shown in table \ref{table:sota_cirr}, on the CIRR dataset, our method achieved the state-of-the-art results in all metrics except for Recall@50. As shown in table \ref{table:sota_fiq}, on the FashionIQ dataset, our performance on average Recall@50 exceeds the current SOTA CompoDiff, but it is trained on 18M triplet data, which is hundreds of times larger than our dataset.

\begin{table}
\centering
\footnotesize
\setlength{\tabcolsep}{0.12cm}
\begin{tabular}{c c|c|c|c|c|c|c|c}
\hline
 \multicolumn{2}{c|}{~}&
 \multicolumn{4}{c|}{\text{$\rm Recall@K$}}& 
 \multicolumn{3}{c}{\text{$\rm Recall_{Subset}@K$}} \\
 Method& \# training triplets & K=1& K=5& K=10& K=50& K=1& K=2& K=3\\
 \hline 
 \multicolumn{9}{c}{\text{Supervised}}\\
 \hline
 CLRPLANT w/OSCAR~\cite{liu2021image}\fontsize{4pt}
 %28225
 {\baselineskip}\selectfont{ICCV’2021} &28k& 19.55 & 52.55 & 68.39 & 92.38 & 39.20 & 63.03 & 79.49\\ 
 ARTEMIS~\cite{delmas2022artemis}\fontsize{4pt}{\baselineskip}\selectfont{ICLR’2022} &28k &16.96& 46.10 & 61.31 & 87.73 & 39.99 & 62.20 & 75.67 \\
 CLIP4CIR~\cite{baldrati2022conditioned}\fontsize{4pt}{\baselineskip}\selectfont{CVPRW’2022}&28k&38.53&69.98 &81.86 &95.93 &68.19&85.64 &94.17\\
 BLIP4CIR+Bi~\cite{liu2023bi}\fontsize{4pt}{\baselineskip}\selectfont{arXiv’2023}&28k&40.15&73.08&83.88&96.27&72.10&88.27&95.93\\
 CASE~\cite{levy2023data}\fontsize{4pt}{\baselineskip}\selectfont{arXiv’2023} &28k&48.00 & 79.11 & 87.25 & 97.57 & 75.88 & 90.58 & 96.00\\ 
 \hline
\multicolumn{9}{c}{\text{Zero-shot}}\\
\hline
 Pic2Word~\cite{saito2023pic2word}\fontsize{4pt}{\baselineskip}\selectfont{CVPR’2023} &-& 23.90 & 51.70 & 65.30 & 87.80 & - & - & -\\ 
 PALAVRA~\cite{cohen2022my}\fontsize{4pt}{\baselineskip}\selectfont{ECCV’2022} &-& 16.62 & 43.49 & 58.51 & 83.95 & 41.61 & 65.30 & 80.94\\
 SEARLE-XL~\cite{baldrati2023zero}\fontsize{4pt}{\baselineskip}\selectfont{arXiv’2023} &-&24.22 &52.41 &66.29 &88.63&53.71 &74.63 &87.61\\
 CompoDiff w/T5-XL~\cite{gu2023compodiff}\fontsize{4pt}{\baselineskip}\selectfont{arXiv’2023}&18m&19.37 &53.81 &72.02 &90.85&28.96 &49.21 &67.03\\
 CASE Pre-LaSCo.Ca.~\cite{levy2023data}\fontsize{4pt}{\baselineskip}\selectfont{arXiv’2023} &\textasciitilde 360k& 35.40 & 65.78 & 78.53 & \textbf{94.63} & 64.29 & 82.66 & 91.61\\ 
 \hline
 \textbf{Template-based} & 16k&\textbf{38.43} & \textbf{68.92} & \textbf{79.93} & 94.05 & \textbf{68.60} & \textbf{85.61} & \textbf{93.93}\\ 
 % \textbf{LLM-based (T5)} &32k& 36.53 & 67.59 & 79.13 & 94.36 & 64.72 & 82.80 & 92.22\\ 
 \textbf{LLM-based (ChatGPT)} &15k& 36.82 & 66.65 & 78.55 & 93.57 & 64.60 & 82.94 & 92.27\\ 
 \hline
\end{tabular}
\vspace{5pt}
\caption{Comparision on CIRR test set.}
\label{table:sota_cirr}
\end{table}


\begin{table}
\begin{scriptsize}
\setlength{\tabcolsep}{0.12cm}
\centering
\begin{tabular}{c c|c c|c c|c c|c c}
\hline
 \multicolumn{2}{c|}{~}&
 \multicolumn{2}{c|}{Shirt}& 
 \multicolumn{2}{c|}{Dress}& 
 \multicolumn{2}{c|}{TopTee}&
 \multicolumn{2}{c}{Average}\\
 Method& \# training triplets & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50} & \text{R@10} & \text{R@50}\\
 \hline
 \multicolumn{10}{c}{Supervised}\\
 \hline
 CLRPLANT w/OSCAR~\cite{liu2021image}\fontsize{4pt}{\baselineskip}\selectfont{ICCV’2021} &18k& 17.53 & 38.81 & 17.45 & 40.41 & 21.64 & 45.38 & 18.87& 41.53\\ 
 ARTEMIS~\cite{delmas2022artemis}\fontsize{4pt}{\baselineskip}\selectfont{ICLR’2022}&18k&21.78&43.64&27.16&52.40&29.20&54.83&26.05&50.29\\
CLIP4CIR~\cite{baldrati2022conditioned}\fontsize{4pt}{\baselineskip}\selectfont{CVPRW’2022} &18k&39.99 &60.45&33.81 &59.40&41.41 &65.37 &38.32&61.74\\
 BLIP4CIR+Bi~\cite{liu2023bi}\fontsize{4pt}{\baselineskip}\selectfont{arXiv’2023}&18k&41.76 &64.28&42.09 &67.33&46.61 &70.32&43.49& 67.31\\
 CASE~\cite{levy2023data}\fontsize{4pt}{\baselineskip}\selectfont{arXiv’2023} &18k&48.48 &70.23&47.44 &69.36&50.18 &72.24 &48.79& 70.68\\
 \hline
 \multicolumn{10}{c}{Zero-shot}\\
 \hline
 Pic2Word~\cite{saito2023pic2word}\fontsize{4pt}{\baselineskip}\selectfont{CVPR’2023} &-& 26.20 & 43.60 & 20.00 & 40.20 & 27.90 & 47.40 & 24.70& 43.70\\ 
 PALAVRA~\cite{cohen2022my}\fontsize{4pt}{\baselineskip}\selectfont{ECCV’2022}&-&21.49&37.05&17.25&35.94&20.55&38.76&19.76&37.25\\
 SEARLE-XL-OTI~\cite{baldrati2023zero}\fontsize{4pt}{\baselineskip}\selectfont{arXiv’2023} &-&30.37 &47.49&21.57 &44.47&30.90 &51.76 &27.61& 47.90\\
 CompoDiff w/T5-XL~\cite{gu2023compodiff}\fontsize{4pt}{\baselineskip}\selectfont{arXiv’2023} &18m&\textbf{38.10} &\textbf{52.48}&\textbf{33.91} &47.85&\textbf{40.07} &52.22 &\textbf{37.36}& 50.85\\
 \hline
 \textbf{Template-based} &16k&32.83 &52.40 &27.86 &\textbf{49.48}&35.24&57.42&31.98&53.10\\
 % \textbf{LLM-based(T5)} &32k&32.73 &\textbf{53.48} &27.76 &\textbf{51.22}&37.18 &\textbf{59.46}&32.56&\textbf{54.72}\\
 \textbf{LLM-based(ChatGPT)} &15k&32.34 &52.06 &28.90 &49.43&36.56 &\textbf{58.49}&32.60&\textbf{53.33}\\
 \hline
\end{tabular}
\caption{Comparasion on FashionIQ validation set.}
\label{table:sota_fiq}
\end{scriptsize}
\end{table}


\subsection{Qualitative Results}
In figure \ref{fig:qualitative_results}, we show the qualitative results for our model on zero-shot composed image retrieval. specifically, each row includes reference image, relative caption and the top five images retrieved, where the ground truth is marked with a green box. The results demonstrate the effectiveness of our proposed method in successfully retrieving the target image.

\begin{figure}
    \centering
    \includegraphics[width=12cm]{images/visualize1.png}
    \caption{Qualitative results on CIRR. From left to right are the reference image, relative caption and the top five images retrieved, among which the ground truth is marked with a green box.}
    \label{fig:qualitative_results}
\end{figure}







% \begin{table}
% \centering
% \scriptsize
% \begin{tabular}{c c||c|c|c|c|c|c|c}
% \hline
%  \multicolumn{2}{c||}{~}&
%  \multicolumn{4}{c|}{\text{$Recall@K$}}& 
%  \multicolumn{3}{c}{\text{$Recall_{Subset}@K$}} \\
%  Method& Num of training triplets & K=1& K=5& K=10& K=50& K=1& K=2& K=3\\
%  \hline \hline
%  Pic2Word~\cite{saito2023pic2word}\tiny{CVPR’2023} &-& 23.90 & 51.70 & 65.30 & 87.80 & - & - & -\\ 
%  PALAVRA~\cite{cohen2022my}\tiny{ECCV’2022} &-& 16.62 & 43.49 & 58.51 & 83.95 & 41.61 & 65.30 & 80.94\\
%  SEARLE-XL~\cite{baldrati2023zero}\tiny{arXiv’2023} &-&24.22 &52.41 &66.29 &88.63&53.71 &74.63 &87.61\\
%  CompoDiff w/T5-XL~\cite{gu2023compodiff}\tiny{arXiv’2023}&18M&19.37 &53.81 &72.02 &90.85&28.96 &49.21 &67.03\\
%  CASE Pre-LaSCo.Ca.~\cite{levy2023data}\tiny{arXiv’2023} &\textasciitilde 360K& 35.40 & 65.78 & 78.53 & \textbf{94.63} & 64.29 & 82.66 & 91.61\\ 
%  \hline
%  \textbf{Template-based} & 16000&\textbf{38.43} & \textbf{68.92} & \textbf{79.93} & 94.05 & \textbf{68.60} & \textbf{85.61} & \textbf{93.93}\\ 
%  \textbf{Language Model-based} &32222& 36.53 & 67.59 & 79.13 & 94.36 & 64.72 & 82.80 & 92.22\\ 
%  \textbf{ChatGPT-based} &15033& 36.82 & 66.65 & 78.55 & 93.57 & 64.60 & 82.94 & 92.27\\ 
%  \hline
% \end{tabular}
% \caption{Comparision on CIRR test set. \weidi{give citation for methods in the table, add another column on the whether these methods have been published, for example, arxiv ? and add column for how muchd data the model is used for training.}}
% \label{table:sota_cirr}
% \end{table}
